Measurement of the Differential and Total Cross Sections of the ${\gamma}d \to K^0 {\Lambda} (p)$ Reaction within the Resonance Region

We report the first measurement of differential and total cross sections for the ${\gamma}d \to K^0{\Lambda}(p)$ reaction, using data from the CLAS detector at the Thomas Jefferson National Accelerator Facility. Data collected during two separate experimental runs were studied with photon-energy coverage 0.8 - 3.6 GeV and 0.5 - 2.6 GeV, respectively. The two measurements are consistent giving confidence in the method and determination of systematic uncertainties. The cross sections are compared with predictions from the KAON-MAID theoretical model (without kaon exchange), which deviate from the data at higher W and at forward kaon angles. These data, along with previously published cross sections for $K^+ {\Lambda}$ photoproduction, provide essential constraints on the nucleon resonance spectrum. A first partial wave analysis has been performed that describes the data without the introduction of new resonances.

==> g10table.tex <==
\begin{table*}[tbh]
\centering
\caption{The differential cross section from g10 dataset with beam energies between 1.00 and 2.00. All energies in the table have units of GeV and cross sections have units of $\mu b$.}
\label{tab:diffcrossg13}
\begin{sideways}
\resizebox{9.0in}{!}{
\begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|c||c|c|c|c|c|c|} \hline
\boldmath$E_\gamma$ &\boldmath$W$ &\boldmath$\cos\theta_{CM}^{K^{0}}$ &\boldmath$\frac{d\sigma}{dcos\theta_{CM}^{K^{0}}}$ &\boldmath$\sigma_{stat}$ &\boldmath$\sigma_{syst}$ &\boldmath$E_\gamma$ &\boldmath$W$ &\boldmath$\cos\theta_{CM}^{K^{0}}$ &\boldmath$\frac{d\sigma}{dcos\theta_{CM}^{K^{0}}}$ &\boldmath$\sigma_{stat}$ &\boldmath$\sigma_{syst}$ &\boldmath\boldmath$E_\gamma$ &\boldmath\boldmath$W$ &\boldmath\boldmath$\cos\theta_{CM}^{K^{0}}$ &\boldmath\boldmath$\frac{d\sigma}{dcos\theta_{CM}^{K^{0}}}$  &\boldmath\boldmath$\sigma_{stat}$ &\boldmath$\sigma_{syst}$ \\ \hline
1.10 & 1.718 & -0.65 & 1.0001 & 0.3920 & 0.1000 & 1.30 & 1.824 & 0.15 & 0.5860 & 0.0468 & 0.0586 & 1.70 & 2.019 & -0.25 & 0.0931 & 0.0180 & 0.0093 \\ \hline
1.10 & 1.718 & -0.55 & 1.2259 & 0.2744 & 0.1226 & 1.30 & 1.824 & 0.25 & 0.6222 & 0.0507 & 0.0622 & 1.70 & 2.019 & -0.15 & 0.1031 & 0.0154 & 0.0103 \\ \hline
1.10 & 1.718 & -0.45 & 0.7197 & 0.1866 & 0.0720 & 1.30 & 1.824 & 0.35 & 0.6077 & 0.0469 & 0.0608 & 1.70 & 2.019 & -0.05 & 0.1202 & 0.0152 & 0.0120 \\ \hline
1.10 & 1.718 & -0.35 & 0.7835 & 0.1420 & 0.0784 & 1.30 & 1.824 & 0.55 & 0.7011 & 0.0683 & 0.0701 & 1.70 & 2.019 & 0.15 & 0.1841 & 0.0169 & 0.0184 \\ \hline
1.10 & 1.718 & -0.25 & 0.8272 & 0.1275 & 0.0827 & 1.30 & 1.824 & 0.65 & 0.5657 & 0.0704 & 0.0566 & 1.70 & 2.019 & 0.25 & 0.2860 & 0.0211 & 0.0286 \\ \hline
1.10 & 1.718 & -0.15 & 0.7251 & 0.1002 & 0.0725 & 1.30 & 1.824 & 0.75 & 0.4874 & 0.0939 & 0.0487 & 1.70 & 2.019 & 0.35 & 0.2997 & 0.0214 & 0.0300 \\ \hline
1.10 & 1.718 & -0.05 & 0.7705 & 0.0967 & 0.0770 & 1.50 & 1.924 & -0.65 & 0.4431 & 0.1668 & 0.0443 & 1.70 & 2.019 & 0.45 & 0.3424 & 0.0265 & 0.0342 \\ \hline
1.10 & 1.718 & 0.05 & 0.5238 & 0.0833 & 0.0524 & 1.50 & 1.924 & -0.55 & 0.3014 & 0.0827 & 0.0301 & 1.70 & 2.019 & 0.55 & 0.4081 & 0.0328 & 0.0408 \\ \hline
1.10 & 1.718 & 0.15 & 0.5988 & 0.0777 & 0.0599 & 1.50 & 1.924 & -0.45 & 0.1858 & 0.0423 & 0.0186 & 1.70 & 2.019 & 0.65 & 0.4976 & 0.0439 & 0.0498 \\ \hline
1.10 & 1.718 & 0.25 & 0.6063 & 0.0846 & 0.0606 & 1.50 & 1.924 & -0.35 & 0.1970 & 0.0309 & 0.0197 & 1.70 & 2.019 & 0.75 & 0.3675 & 0.0552 & 0.0367 \\ \hline
1.10 & 1.718 & 0.35 & 0.6631 & 0.0796 & 0.0663 & 1.50 & 1.924 & -0.25 & 0.2266 & 0.0297 & 0.0227 & 1.90 & 2.110 & -0.55 & 0.1104 & 0.0372 & 0.0110 \\ \hline
1.10 & 1.718 & 0.45 & 0.6160 & 0.0901 & 0.0616 & 1.50 & 1.924 & -0.15 & 0.2470 & 0.0280 & 0.0247 & 1.90 & 2.110 & -0.45 & 0.0570 & 0.0184 & 0.0057 \\ \hline
1.10 & 1.718 & 0.55 & 0.3775 & 0.0875 & 0.0377 & 1.50 & 1.924 & -0.05 & 0.2370 & 0.0252 & 0.0237 & 1.90 & 2.110 & -0.35 & 0.1054 & 0.0178 & 0.0105 \\ \hline
1.10 & 1.718 & 0.65 & 0.3148 & 0.1023 & 0.0315 & 1.50 & 1.924 & 0.05 & 0.2997 & 0.0263 & 0.0300 & 1.90 & 2.110 & -0.25 & 0.0980 & 0.0135 & 0.0098 \\ \hline
1.10 & 1.718 & 0.75 & 0.2362 & 0.1079 & 0.0236 & 1.50 & 1.924 & 0.15 & 0.2525 & 0.0244 & 0.0253 & 1.90 & 2.110 & -0.15 & 0.0576 & 0.0111 & 0.0058 \\ \hline
1.30 & 1.824 & -0.65 & 0.8499 & 0.2805 & 0.0850 & 1.50 & 1.924 & 0.25 & 0.3553 & 0.0282 & 0.0355 & 1.90 & 2.110 & -0.05 & 0.0593 & 0.0121 & 0.0059 \\ \hline
1.30 & 1.824 & -0.55 & 0.8877 & 0.1759 & 0.0888 & 1.50 & 1.924 & 0.35 & 0.3929 & 0.0305 & 0.0393 & 1.90 & 2.110 & 0.05 & 0.0992 & 0.0129 & 0.0099 \\ \hline
1.30 & 1.824 & -0.45 & 0.6927 & 0.0975 & 0.0693 & 1.50 & 1.924 & 0.45 & 0.4366 & 0.0343 & 0.0437 & 1.90 & 2.110 & 0.15 & 0.1265 & 0.0132 & 0.0126 \\ \hline
1.30 & 1.824 & -0.35 & 0.5746 & 0.0660 & 0.0575 & 1.50 & 1.924 & 0.55 & 0.4531 & 0.0411 & 0.0453 & 1.90 & 2.110 & 0.25 & 0.1438 & 0.0151 & 0.0144 \\ \hline
1.30 & 1.824 & -0.25 & 0.5950 & 0.0587 & 0.0595 & 1.50 & 1.924 & 0.65 & 0.3842 & 0.0445 & 0.0384 & 1.90 & 2.110 & 0.35 & 0.1976 & 0.0179 & 0.0198 \\ \hline
1.30 & 1.824 & -0.15 & 0.5350 & 0.0506 & 0.0535 & 1.50 & 1.924 & 0.75 & 0.3531 & 0.0594 & 0.0353 & 1.90 & 2.110 & 0.45 & 0.2123 & 0.0187 & 0.0212 \\ \hline
1.30 & 1.824 & -0.05 & 0.7102 & 0.0466 & 0.0710 & 1.70 & 2.019 & -0.55 & 0.1506 & 0.0542 & 0.0151 & 1.90 & 2.110 & 0.55 & 0.3304 & 0.0286 & 0.0330 \\ \hline
1.30 & 1.824 & 0.05 & 0.6092 & 0.0468 & 0.0609 & 1.70 & 2.019 & -0.45 & 0.1134 & 0.0272 & 0.0113 & 1.90 & 2.110 & 0.65 & 0.4143 & 0.0398 & 0.0414 \\ \hline
1.30 & 1.824 & 0.15 & 0.5860 & 0.0468 & 0.0586 &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\end{tabular}}
\end{sideways}
\end{table*}


\begin{table*}[tbh]
\centering
\caption{The differential cross section from g10 dataset with beam energies between 2.00 and 3.00. All energies in the table have units of GeV and cross sections have units of $\mu b$.}
\label{tab:diffcrossg13}
\begin{sideways}
\resizebox{9.0in}{!}{
\begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|c||c|c|c|c|c|c|} \hline
\boldmath$E_\gamma$ &\boldmath$W$ &\boldmath$\cos\theta_{CM}^{K^{0}}$ &\boldmath$\frac{d\sigma}{dcos\theta_{CM}^{K^{0}}}$ &\boldmath$\sigma_{stat}$ &\boldmath$\sigma_{syst}$ &\boldmath$E_\gamma$ &\boldmath$W$ &\boldmath$\cos\theta_{CM}^{K^{0}}$ &\boldmath$\frac{d\sigma}{dcos\theta_{CM}^{K^{0}}}$ &\boldmath$\sigma_{stat}$ &\boldmath$\sigma_{syst}$ &\boldmath\boldmath$E_\gamma$ &\boldmath\boldmath$W$ &\boldmath\boldmath$\cos\theta_{CM}^{K^{0}}$ &\boldmath\boldmath$\frac{d\sigma}{dcos\theta_{CM}^{K^{0}}}$  &\boldmath\boldmath$\sigma_{stat}$ &\boldmath$\sigma_{syst}$ \\ \hline
2.10 & 2.198 & -0.55 & 0.0599 & 0.0326 & 0.0060 & 2.30 & 2.281 & 0.25 & 0.0688 & 0.0091 & 0.0069 & 2.70 & 2.441 & -0.25 & 0.0087 & 0.0049 & 0.0009 \\ \hline
2.10 & 2.198 & -0.45 & 0.0250 & 0.0168 & 0.0025 & 2.30 & 2.281 & 0.35 & 0.1042 & 0.0119 & 0.0104 & 2.70 & 2.441 & -0.15 & 0.0053 & 0.0037 & 0.0005 \\ \hline
2.10 & 2.198 & -0.35 & 0.0449 & 0.0110 & 0.0045 & 2.30 & 2.281 & 0.45 & 0.1492 & 0.0150 & 0.0149 & 2.70 & 2.441 & -0.05 & 0.0069 & 0.0041 & 0.0007 \\ \hline
2.10 & 2.198 & -0.25 & 0.0405 & 0.0093 & 0.0040 & 2.30 & 2.281 & 0.55 & 0.1856 & 0.0193 & 0.0186 & 2.70 & 2.441 & 0.05 & 0.0056 & 0.0046 & 0.0006 \\ \hline
2.10 & 2.198 & -0.15 & 0.0357 & 0.0084 & 0.0036 & 2.30 & 2.281 & 0.65 & 0.2370 & 0.0251 & 0.0237 & 2.70 & 2.441 & 0.15 & 0.0153 & 0.0052 & 0.0015 \\ \hline
2.10 & 2.198 & -0.05 & 0.0405 & 0.0083 & 0.0040 & 2.30 & 2.281 & 0.75 & 0.2827 & 0.0431 & 0.0283 & 2.70 & 2.441 & 0.25 & 0.0258 & 0.0063 & 0.0026 \\ \hline
2.10 & 2.198 & 0.05 & 0.0285 & 0.0085 & 0.0029 & 2.50 & 2.362 & -0.55 & 0.0451 & 0.0201 & 0.0045 & 2.70 & 2.441 & 0.35 & 0.0614 & 0.0095 & 0.0061 \\ \hline
2.10 & 2.198 & 0.15 & 0.0647 & 0.0102 & 0.0065 & 2.50 & 2.362 & -0.45 & 0.0303 & 0.0100 & 0.0030 & 2.70 & 2.441 & 0.45 & 0.0758 & 0.0114 & 0.0076 \\ \hline
2.10 & 2.198 & 0.35 & 0.1253 & 0.0136 & 0.0125 & 2.50 & 2.362 & -0.35 & 0.0144 & 0.0067 & 0.0014 & 2.70 & 2.441 & 0.55 & 0.0908 & 0.0128 & 0.0091 \\ \hline
2.10 & 2.198 & 0.45 & 0.1790 & 0.0166 & 0.0179 & 2.50 & 2.362 & -0.25 & 0.0140 & 0.0055 & 0.0014 & 2.70 & 2.441 & 0.65 & 0.1389 & 0.0185 & 0.0139 \\ \hline
2.10 & 2.198 & 0.55 & 0.2761 & 0.0232 & 0.0276 & 2.50 & 2.362 & -0.15 & 0.0157 & 0.0054 & 0.0016 & 2.70 & 2.441 & 0.75 & 0.1751 & 0.0357 & 0.0175 \\ \hline
2.10 & 2.198 & 0.65 & 0.3291 & 0.0313 & 0.0329 & 2.50 & 2.362 & -0.05 & 0.0115 & 0.0037 & 0.0011 & 2.90 & 2.516 & -0.55 & 0.0230 & 0.0146 & 0.0023 \\ \hline
2.10 & 2.198 & 0.75 & 0.4658 & 0.0596 & 0.0466 & 2.50 & 2.362 & 0.05 & 0.0100 & 0.0057 & 0.0010 & 2.90 & 2.516 & -0.35 & 0.0168 & 0.0055 & 0.0017 \\ \hline
2.30 & 2.281 & -0.55 & 0.0939 & 0.0263 & 0.0094 & 2.50 & 2.362 & 0.15 & 0.0283 & 0.0073 & 0.0028 & 2.90 & 2.516 & -0.25 & 0.0097 & 0.0038 & 0.0010 \\ \hline
2.30 & 2.281 & -0.45 & 0.0397 & 0.0143 & 0.0040 & 2.50 & 2.362 & 0.25 & 0.0483 & 0.0082 & 0.0048 & 2.90 & 2.516 & 0.05 & 0.0036 & 0.0022 & 0.0004 \\ \hline
2.30 & 2.281 & -0.35 & 0.0160 & 0.0085 & 0.0016 & 2.50 & 2.362 & 0.35 & 0.0763 & 0.0105 & 0.0076 & 2.90 & 2.516 & 0.15 & 0.0102 & 0.0028 & 0.0010 \\ \hline
2.30 & 2.281 & -0.25 & 0.0310 & 0.0077 & 0.0031 & 2.50 & 2.362 & 0.45 & 0.1166 & 0.0132 & 0.0117 & 2.90 & 2.516 & 0.25 & 0.0101 & 0.0040 & 0.0010 \\ \hline
2.30 & 2.281 & -0.15 & 0.0140 & 0.0063 & 0.0014 & 2.50 & 2.362 & 0.55 & 0.1736 & 0.0197 & 0.0174 & 2.90 & 2.516 & 0.35 & 0.0295 & 0.0054 & 0.0029 \\ \hline
2.30 & 2.281 & -0.05 & 0.0165 & 0.0061 & 0.0016 & 2.50 & 2.362 & 0.65 & 0.2240 & 0.0258 & 0.0224 & 2.90 & 2.516 & 0.45 & 0.0428 & 0.0070 & 0.0043 \\ \hline
2.30 & 2.281 & 0.05 & 0.0272 & 0.0063 & 0.0027 & 2.50 & 2.362 & 0.75 & 0.2969 & 0.0454 & 0.0297 & 2.90 & 2.516 & 0.55 & 0.0490 & 0.0087 & 0.0049 \\ \hline
2.30 & 2.281 & 0.15 & 0.0322 & 0.0067 & 0.0032 & 2.70 & 2.441 & -0.45 & 0.0137 & 0.0110 & 0.0014 & 2.90 & 2.516 & 0.65 & 0.0814 & 0.0138 & 0.0081 \\ \hline
2.30 & 2.281 & 0.25 & 0.0688 & 0.0091 & 0.0069 &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\end{tabular}}
\end{sideways}
\end{table*}




==> g13table.tex <==
\begin{table*}[tbh]
\centering
\caption{The differential cross section from g13 dataset with beam energies between 0.90 and 1.60. All energies in the table have units of GeV and cross sections have units of $\mu b$.}
\label{tab:diffcrossg13}
\begin{sideways}
\resizebox{9.0in}{!}{
\begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|c||c|c|c|c|c|c|} \hline
\boldmath$E_\gamma$ &\boldmath$W$ &\boldmath$\cos\theta_{CM}^{K^{0}}$ &\boldmath$\frac{d\sigma}{dcos\theta_{CM}^{K^{0}}}$ &\boldmath$\sigma_{stat}$ &\boldmath$\sigma_{syst}$ &\boldmath$E_\gamma$ &\boldmath$W$ &\boldmath$\cos\theta_{CM}^{K^{0}}$ &\boldmath$\frac{d\sigma}{dcos\theta_{CM}^{K^{0}}}$ &\boldmath$\sigma_{stat}$ &\boldmath$\sigma_{syst}$ &\boldmath\boldmath$E_\gamma$ &\boldmath\boldmath$W$ &\boldmath\boldmath$\cos\theta_{CM}^{K^{0}}$ &\boldmath\boldmath$\frac{d\sigma}{dcos\theta_{CM}^{K^{0}}}$  &\boldmath\boldmath$\sigma_{stat}$ &\boldmath$\sigma_{syst}$ \\ \hline
0.97 & 1.645 & -0.65 & 0.7526 & 0.3508 & 0.0687 & 1.15 & 1.745 & -0.15 & 0.7160 & 0.0494 & 0.0504 & 1.35 & 1.849 & 0.25 & 0.5868 & 0.0322 & 0.0385 \\ \hline
0.97 & 1.645 & -0.55 & 0.7716 & 0.3347 & 0.0704 & 1.15 & 1.745 & -0.05 & 0.7593 & 0.0468 & 0.0535 & 1.35 & 1.849 & 0.35 & 0.5275 & 0.0314 & 0.0346 \\ \hline
0.97 & 1.645 & -0.45 & 0.8650 & 0.2401 & 0.0789 & 1.15 & 1.745 & 0.05 & 0.7495 & 0.0450 & 0.0528 & 1.35 & 1.849 & 0.45 & 0.5636 & 0.0344 & 0.0369 \\ \hline
0.97 & 1.645 & -0.35 & 0.7499 & 0.1734 & 0.0684 & 1.15 & 1.745 & 0.15 & 0.6368 & 0.0398 & 0.0449 & 1.35 & 1.849 & 0.55 & 0.5709 & 0.0393 & 0.0374 \\ \hline
0.97 & 1.645 & -0.25 & 0.7237 & 0.1707 & 0.0660 & 1.15 & 1.745 & 0.25 & 0.7614 & 0.0430 & 0.0536 & 1.35 & 1.849 & 0.65 & 0.5960 & 0.0450 & 0.0391 \\ \hline
0.97 & 1.645 & -0.15 & 0.5918 & 0.1179 & 0.0540 & 1.15 & 1.745 & 0.35 & 0.6695 & 0.0420 & 0.0472 & 1.35 & 1.849 & 0.75 & 0.6750 & 0.0603 & 0.0442 \\ \hline
0.97 & 1.645 & -0.05 & 0.7080 & 0.1100 & 0.0646 & 1.15 & 1.745 & 0.45 & 0.6739 & 0.0434 & 0.0475 & 1.45 & 1.899 & -0.55 & 0.4867 & 0.0716 & 0.0317 \\ \hline
0.97 & 1.645 & 0.05 & 0.7810 & 0.1106 & 0.0713 & 1.15 & 1.745 & 0.55 & 0.6945 & 0.0495 & 0.0489 & 1.45 & 1.899 & -0.45 & 0.5222 & 0.0500 & 0.0346 \\ \hline
0.97 & 1.645 & 0.15 & 0.6485 & 0.1041 & 0.0592 & 1.15 & 1.745 & 0.65 & 0.7114 & 0.0528 & 0.0501 & 1.45 & 1.899 & -0.35 & 0.4060 & 0.0366 & 0.0265 \\ \hline
0.97 & 1.645 & 0.25 & 0.5731 & 0.0938 & 0.0523 & 1.15 & 1.745 & 0.75 & 0.7098 & 0.0662 & 0.0500 & 1.45 & 1.899 & -0.25 & 0.3543 & 0.0293 & 0.0231 \\ \hline
0.97 & 1.645 & 0.35 & 0.5795 & 0.0974 & 0.0529 & 1.25 & 1.798 & -0.65 & 1.4187 & 0.1828 & 0.0956 & 1.45 & 1.899 & -0.15 & 0.3707 & 0.0273 & 0.0242 \\ \hline
0.97 & 1.645 & 0.45 & 0.7046 & 0.1075 & 0.0643 & 1.25 & 1.798 & -0.55 & 1.0263 & 0.1070 & 0.0691 & 1.45 & 1.899 & -0.05 & 0.4015 & 0.0263 & 0.0262 \\ \hline
0.97 & 1.645 & 0.55 & 0.4468 & 0.0961 & 0.0408 & 1.25 & 1.798 & -0.45 & 0.9201 & 0.0788 & 0.0620 & 1.45 & 1.899 & 0.05 & 0.3724 & 0.0241 & 0.0243 \\ \hline
0.97 & 1.645 & 0.65 & 0.5162 & 0.1203 & 0.0471 & 1.25 & 1.798 & -0.35 & 0.8025 & 0.0582 & 0.0541 & 1.45 & 1.899 & 0.15 & 0.3534 & 0.0246 & 0.0230 \\ \hline
0.97 & 1.645 & 0.75 & 0.5183 & 0.1444 & 0.0473 & 1.25 & 1.798 & -0.25 & 0.7676 & 0.0502 & 0.0517 & 1.45 & 1.899 & 0.25 & 0.3556 & 0.0246 & 0.0232 \\ \hline
1.05 & 1.690 & -0.55 & 1.3388 & 0.2333 & 0.1022 & 1.25 & 1.798 & -0.15 & 0.7017 & 0.0432 & 0.0473 & 1.45 & 1.899 & 0.35 & 0.4252 & 0.0264 & 0.0277 \\ \hline
1.05 & 1.690 & -0.45 & 1.0565 & 0.1246 & 0.0807 & 1.25 & 1.798 & -0.05 & 0.7280 & 0.0409 & 0.0490 & 1.45 & 1.899 & 0.45 & 0.5243 & 0.0309 & 0.0342 \\ \hline
1.05 & 1.690 & -0.35 & 1.0600 & 0.1003 & 0.0810 & 1.25 & 1.798 & 0.05 & 0.6225 & 0.0362 & 0.0419 & 1.45 & 1.899 & 0.55 & 0.5309 & 0.0350 & 0.0346 \\ \hline
1.05 & 1.690 & -0.25 & 0.8664 & 0.0860 & 0.0662 & 1.25 & 1.798 & 0.15 & 0.6545 & 0.0382 & 0.0441 & 1.45 & 1.899 & 0.65 & 0.5028 & 0.0386 & 0.0328 \\ \hline
1.05 & 1.690 & -0.15 & 0.8887 & 0.0752 & 0.0679 & 1.25 & 1.798 & 0.25 & 0.7707 & 0.0397 & 0.0519 & 1.45 & 1.899 & 0.75 & 0.6113 & 0.0560 & 0.0398 \\ \hline
1.05 & 1.690 & -0.05 & 0.8245 & 0.0660 & 0.0630 & 1.25 & 1.798 & 0.35 & 0.7776 & 0.0393 & 0.0524 & 1.55 & 1.948 & -0.55 & 0.2888 & 0.0511 & 0.0196 \\ \hline
1.05 & 1.690 & 0.05 & 0.8251 & 0.0625 & 0.0630 & 1.25 & 1.798 & 0.45 & 0.7207 & 0.0407 & 0.0486 & 1.55 & 1.948 & -0.45 & 0.2433 & 0.0322 & 0.0163 \\ \hline
1.05 & 1.690 & 0.15 & 0.7596 & 0.0588 & 0.0580 & 1.25 & 1.798 & 0.55 & 0.6272 & 0.0432 & 0.0423 & 1.55 & 1.948 & -0.35 & 0.2031 & 0.0231 & 0.0136 \\ \hline
1.05 & 1.690 & 0.25 & 0.7743 & 0.0599 & 0.0591 & 1.25 & 1.798 & 0.65 & 0.6782 & 0.0486 & 0.0457 & 1.55 & 1.948 & -0.25 & 0.1967 & 0.0198 & 0.0132 \\ \hline
1.05 & 1.690 & 0.35 & 0.6727 & 0.0578 & 0.0514 & 1.25 & 1.798 & 0.75 & 0.6865 & 0.0619 & 0.0462 & 1.55 & 1.948 & -0.15 & 0.1837 & 0.0176 & 0.0123 \\ \hline
1.05 & 1.690 & 0.45 & 0.7107 & 0.0601 & 0.0543 & 1.35 & 1.849 & -0.65 & 0.7907 & 0.1461 & 0.0518 & 1.55 & 1.948 & -0.05 & 0.1769 & 0.0169 & 0.0119 \\ \hline
1.05 & 1.690 & 0.55 & 0.5796 & 0.0593 & 0.0443 & 1.35 & 1.849 & -0.55 & 0.7091 & 0.0870 & 0.0465 & 1.55 & 1.948 & 0.05 & 0.2319 & 0.0180 & 0.0156 \\ \hline
1.05 & 1.690 & 0.65 & 0.5546 & 0.0708 & 0.0424 & 1.35 & 1.849 & -0.45 & 0.7009 & 0.0606 & 0.0460 & 1.55 & 1.948 & 0.15 & 0.2772 & 0.0186 & 0.0186 \\ \hline
1.05 & 1.690 & 0.75 & 0.7033 & 0.0966 & 0.0537 & 1.35 & 1.849 & -0.35 & 0.6024 & 0.0468 & 0.0395 & 1.55 & 1.948 & 0.25 & 0.3032 & 0.0189 & 0.0203 \\ \hline
1.15 & 1.745 & -0.65 & 1.1144 & 0.1892 & 0.0785 & 1.35 & 1.849 & -0.25 & 0.5990 & 0.0401 & 0.0393 & 1.55 & 1.948 & 0.35 & 0.3116 & 0.0208 & 0.0209 \\ \hline
1.15 & 1.745 & -0.55 & 1.0891 & 0.1242 & 0.0767 & 1.35 & 1.849 & -0.15 & 0.5643 & 0.0351 & 0.0370 & 1.55 & 1.948 & 0.45 & 0.3239 & 0.0235 & 0.0217 \\ \hline
1.15 & 1.745 & -0.45 & 1.0308 & 0.0892 & 0.0726 & 1.35 & 1.849 & -0.05 & 0.5662 & 0.0326 & 0.0371 & 1.55 & 1.948 & 0.55 & 0.3861 & 0.0283 & 0.0259 \\ \hline
1.15 & 1.745 & -0.35 & 0.8852 & 0.0674 & 0.0624 & 1.35 & 1.849 & 0.05 & 0.5395 & 0.0309 & 0.0354 & 1.55 & 1.948 & 0.65 & 0.4386 & 0.0352 & 0.0294 \\ \hline
1.15 & 1.745 & -0.25 & 0.7947 & 0.0557 & 0.0560 & 1.35 & 1.849 & 0.15 & 0.5472 & 0.0303 & 0.0359 & 1.55 & 1.948 & 0.75 & 0.4330 & 0.0488 & 0.0290 \\ \hline
\end{tabular}}
\end{sideways}
\end{table*}


\begin{table*}[tbh]
\centering
\caption{The differential cross section from g13 dataset with beam energies between 1.60 and 2.10. All energies in the table have units of GeV and cross sections have units of $\mu b$.}
\label{tab:diffcrossg13}
\begin{sideways}
\resizebox{9.0in}{!}{
\begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|c||c|c|c|c|c|c|} \hline
\boldmath$E_\gamma$ &\boldmath$W$ &\boldmath$\cos\theta_{CM}^{K^{0}}$ &\boldmath$\frac{d\sigma}{dcos\theta_{CM}^{K^{0}}}$ &\boldmath$\sigma_{stat}$ &\boldmath$\sigma_{syst}$ &\boldmath$E_\gamma$ &\boldmath$W$ &\boldmath$\cos\theta_{CM}^{K^{0}}$ &\boldmath$\frac{d\sigma}{dcos\theta_{CM}^{K^{0}}}$ &\boldmath$\sigma_{stat}$ &\boldmath$\sigma_{syst}$ &\boldmath\boldmath$E_\gamma$ &\boldmath\boldmath$W$ &\boldmath\boldmath$\cos\theta_{CM}^{K^{0}}$ &\boldmath\boldmath$\frac{d\sigma}{dcos\theta_{CM}^{K^{0}}}$  &\boldmath\boldmath$\sigma_{stat}$ &\boldmath$\sigma_{syst}$ \\ \hline
1.65 & 1.996 & -0.55 & 0.1804 & 0.0355 & 0.0122 & 1.75 & 2.042 & 0.35 & 0.2370 & 0.0173 & 0.0159 & 1.95 & 2.132 & -0.15 & 0.0521 & 0.0091 & 0.0034 \\ \hline
1.65 & 1.996 & -0.45 & 0.1912 & 0.0256 & 0.0124 & 1.75 & 2.042 & 0.45 & 0.2789 & 0.0207 & 0.0187 & 1.95 & 2.132 & -0.05 & 0.0721 & 0.0092 & 0.0047 \\ \hline
1.65 & 1.996 & -0.35 & 0.1592 & 0.0185 & 0.0103 & 1.75 & 2.042 & 0.55 & 0.3534 & 0.0259 & 0.0238 & 1.95 & 2.132 & 0.05 & 0.0786 & 0.0097 & 0.0052 \\ \hline
1.65 & 1.996 & -0.25 & 0.1204 & 0.0156 & 0.0078 & 1.75 & 2.042 & 0.65 & 0.4479 & 0.0370 & 0.0301 & 1.95 & 2.132 & 0.15 & 0.0785 & 0.0105 & 0.0053 \\ \hline
1.65 & 1.996 & -0.15 & 0.1280 & 0.0143 & 0.0083 & 1.75 & 2.042 & 0.75 & 0.6691 & 0.0660 & 0.0449 & 1.95 & 2.132 & 0.25 & 0.1315 & 0.0122 & 0.0086 \\ \hline
1.65 & 1.996 & -0.05 & 0.1266 & 0.0139 & 0.0083 & 1.85 & 2.088 & -0.55 & 0.0601 & 0.0203 & 0.0041 & 1.95 & 2.132 & 0.35 & 0.1550 & 0.0135 & 0.0102 \\ \hline
1.65 & 1.996 & 0.05 & 0.1547 & 0.0150 & 0.0100 & 1.85 & 2.088 & -0.45 & 0.0887 & 0.0160 & 0.0059 & 1.95 & 2.132 & 0.45 & 0.2020 & 0.0169 & 0.0132 \\ \hline
1.65 & 1.996 & 0.15 & 0.2031 & 0.0160 & 0.0132 & 1.85 & 2.088 & -0.35 & 0.0908 & 0.0137 & 0.0061 & 1.95 & 2.132 & 0.55 & 0.2525 & 0.0210 & 0.0165 \\ \hline
1.65 & 1.996 & 0.25 & 0.2171 & 0.0169 & 0.0141 & 1.85 & 2.088 & -0.25 & 0.0897 & 0.0114 & 0.0060 & 1.95 & 2.132 & 0.65 & 0.3120 & 0.0320 & 0.0204 \\ \hline
1.65 & 1.996 & 0.35 & 0.2691 & 0.0187 & 0.0175 & 1.85 & 2.088 & -0.15 & 0.0844 & 0.0109 & 0.0056 & 1.95 & 2.132 & 0.75 & 0.3306 & 0.0576 & 0.0216 \\ \hline
1.65 & 1.996 & 0.45 & 0.3208 & 0.0218 & 0.0208 & 1.85 & 2.088 & -0.05 & 0.0809 & 0.0106 & 0.0055 & 2.05 & 2.176 & -0.55 & 0.0818 & 0.0199 & 0.0054 \\ \hline
1.65 & 1.996 & 0.55 & 0.4012 & 0.0282 & 0.0260 & 1.85 & 2.088 & 0.05 & 0.0912 & 0.0104 & 0.0061 & 2.05 & 2.176 & -0.45 & 0.0738 & 0.0123 & 0.0048 \\ \hline
1.65 & 1.996 & 0.65 & 0.4558 & 0.0361 & 0.0296 & 1.85 & 2.088 & 0.15 & 0.1192 & 0.0121 & 0.0080 & 2.05 & 2.176 & -0.35 & 0.0563 & 0.0100 & 0.0037 \\ \hline
1.65 & 1.996 & 0.75 & 0.5720 & 0.0541 & 0.0371 & 1.85 & 2.088 & 0.25 & 0.1362 & 0.0129 & 0.0091 & 2.05 & 2.176 & -0.25 & 0.0519 & 0.0091 & 0.0034 \\ \hline
1.75 & 2.042 & -0.55 & 0.1653 & 0.0319 & 0.0111 & 1.85 & 2.088 & 0.35 & 0.1835 & 0.0147 & 0.0123 & 2.05 & 2.176 & -0.15 & 0.0440 & 0.0084 & 0.0029 \\ \hline
1.75 & 2.042 & -0.45 & 0.1790 & 0.0223 & 0.0120 & 1.85 & 2.088 & 0.45 & 0.2713 & 0.0185 & 0.0181 & 2.05 & 2.176 & -0.05 & 0.0449 & 0.0088 & 0.0029 \\ \hline
1.75 & 2.042 & -0.35 & 0.0932 & 0.0153 & 0.0063 & 1.85 & 2.088 & 0.55 & 0.2775 & 0.0223 & 0.0185 & 2.05 & 2.176 & 0.05 & 0.0411 & 0.0091 & 0.0027 \\ \hline
1.75 & 2.042 & -0.25 & 0.0830 & 0.0129 & 0.0056 & 1.85 & 2.088 & 0.65 & 0.3610 & 0.0329 & 0.0241 & 2.05 & 2.176 & 0.15 & 0.0668 & 0.0095 & 0.0045 \\ \hline
1.75 & 2.042 & -0.15 & 0.0829 & 0.0121 & 0.0056 & 1.85 & 2.088 & 0.75 & 0.4562 & 0.0600 & 0.0305 & 2.05 & 2.176 & 0.25 & 0.1055 & 0.0114 & 0.0070 \\ \hline
1.75 & 2.042 & -0.05 & 0.0866 & 0.0121 & 0.0059 & 1.95 & 2.132 & -0.55 & 0.0789 & 0.0214 & 0.0052 & 2.05 & 2.176 & 0.35 & 0.1462 & 0.0133 & 0.0096 \\ \hline
1.75 & 2.042 & 0.05 & 0.1539 & 0.0138 & 0.0104 & 1.95 & 2.132 & -0.45 & 0.0836 & 0.0146 & 0.0056 & 2.05 & 2.176 & 0.45 & 0.2122 & 0.0165 & 0.0139 \\ \hline
1.75 & 2.042 & 0.15 & 0.1753 & 0.0154 & 0.0118 & 1.95 & 2.132 & -0.35 & 0.0621 & 0.0113 & 0.0041 & 2.05 & 2.176 & 0.55 & 0.2108 & 0.0201 & 0.0138 \\ \hline
1.75 & 2.042 & 0.25 & 0.1615 & 0.0147 & 0.0109 & 1.95 & 2.132 & -0.25 & 0.0672 & 0.0106 & 0.0044 & 2.05 & 2.176 & 0.65 & 0.3170 & 0.0358 & 0.0208 \\ \hline
1.75 & 2.042 & 0.35 & 0.2370 & 0.0173 & 0.0159 & 1.95 & 2.132 & -0.15 & 0.0521 & 0.0091 & 0.0034 &  &  &  &  &  &  \\ \hline
\end{tabular}}
\end{sideways}
\end{table*}


\begin{table*}[tbh]
\centering
\caption{The differential cross section from g13 dataset with beam energies between 2.10 and 2.50. All energies in the table have units of GeV and cross sections have units of $\mu b$.}
\label{tab:diffcrossg13}
\begin{sideways}
\resizebox{9.0in}{!}{
\begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|c||c|c|c|c|c|c|} \hline
\boldmath$E_\gamma$ &\boldmath$W$ &\boldmath$\cos\theta_{CM}^{K^{0}}$ &\boldmath$\frac{d\sigma}{dcos\theta_{CM}^{K^{0}}}$ &\boldmath$\sigma_{stat}$ &\boldmath$\sigma_{syst}$ &\boldmath$E_\gamma$ &\boldmath$W$ &\boldmath$\cos\theta_{CM}^{K^{0}}$ &\boldmath$\frac{d\sigma}{dcos\theta_{CM}^{K^{0}}}$ &\boldmath$\sigma_{stat}$ &\boldmath$\sigma_{syst}$ &\boldmath\boldmath$E_\gamma$ &\boldmath\boldmath$W$ &\boldmath\boldmath$\cos\theta_{CM}^{K^{0}}$ &\boldmath\boldmath$\frac{d\sigma}{dcos\theta_{CM}^{K^{0}}}$  &\boldmath\boldmath$\sigma_{stat}$ &\boldmath$\sigma_{syst}$ \\ \hline
2.15 & 2.219 & -0.55 & 0.0525 & 0.0167 & 0.0036 & 2.25 & 2.261 & -0.35 & 0.0333 & 0.0081 & 0.0023 & 2.35 & 2.302 & 0.25 & 0.0642 & 0.0083 & 0.0042 \\ \hline
2.15 & 2.219 & -0.45 & 0.0488 & 0.0114 & 0.0033 & 2.25 & 2.261 & -0.25 & 0.0242 & 0.0073 & 0.0017 & 2.35 & 2.302 & 0.35 & 0.0991 & 0.0102 & 0.0065 \\ \hline
2.15 & 2.219 & -0.35 & 0.0387 & 0.0091 & 0.0026 & 2.25 & 2.261 & -0.05 & 0.0109 & 0.0062 & 0.0008 & 2.35 & 2.302 & 0.45 & 0.1487 & 0.0139 & 0.0097 \\ \hline
2.15 & 2.219 & -0.25 & 0.0418 & 0.0078 & 0.0028 & 2.25 & 2.261 & 0.05 & 0.0281 & 0.0076 & 0.0019 & 2.35 & 2.302 & 0.55 & 0.1837 & 0.0184 & 0.0120 \\ \hline
2.15 & 2.219 & -0.15 & 0.0217 & 0.0070 & 0.0015 & 2.25 & 2.261 & 0.15 & 0.0231 & 0.0078 & 0.0016 & 2.35 & 2.302 & 0.65 & 0.2135 & 0.0301 & 0.0140 \\ \hline
2.15 & 2.219 & -0.05 & 0.0282 & 0.0073 & 0.0019 & 2.25 & 2.261 & 0.25 & 0.0505 & 0.0092 & 0.0035 & 2.45 & 2.342 & -0.55 & 0.0285 & 0.0131 & 0.0137 \\ \hline
2.15 & 2.219 & 0.05 & 0.0466 & 0.0087 & 0.0031 & 2.25 & 2.261 & 0.35 & 0.1099 & 0.0118 & 0.0076 & 2.45 & 2.342 & -0.45 & 0.0266 & 0.0086 & 0.0018 \\ \hline
2.15 & 2.219 & 0.15 & 0.0408 & 0.0077 & 0.0028 & 2.25 & 2.261 & 0.45 & 0.1491 & 0.0141 & 0.0103 & 2.45 & 2.342 & -0.35 & 0.0155 & 0.0069 & 0.0010 \\ \hline
2.15 & 2.219 & 0.25 & 0.0793 & 0.0097 & 0.0055 & 2.25 & 2.261 & 0.55 & 0.1872 & 0.0199 & 0.0129 & 2.45 & 2.342 & -0.25 & 0.0180 & 0.0065 & 0.0012 \\ \hline
2.15 & 2.219 & 0.35 & 0.1127 & 0.0114 & 0.0076 & 2.25 & 2.261 & 0.65 & 0.3418 & 0.0367 & 0.0236 & 2.45 & 2.342 & -0.15 & 0.0112 & 0.0055 & 0.0009 \\ \hline
2.15 & 2.219 & 0.45 & 0.1409 & 0.0135 & 0.0094 & 2.35 & 2.302 & -0.65 & 0.0367 & 0.0215 & 0.0034 & 2.45 & 2.342 & -0.05 & 0.0063 & 0.0061 & 0.0004 \\ \hline
2.15 & 2.219 & 0.55 & 0.2402 & 0.0200 & 0.0161 & 2.35 & 2.302 & -0.55 & 0.0194 & 0.0111 & 0.0018 & 2.45 & 2.342 & 0.05 & 0.0088 & 0.0063 & 0.0006 \\ \hline
2.15 & 2.219 & 0.65 & 0.2475 & 0.0298 & 0.0166 & 2.35 & 2.302 & -0.45 & 0.0177 & 0.0097 & 0.0012 & 2.45 & 2.342 & 0.15 & 0.0206 & 0.0061 & 0.0014 \\ \hline
2.15 & 2.219 & 0.75 & 0.2573 & 0.0642 & 0.0176 & 2.35 & 2.302 & -0.35 & 0.0260 & 0.0074 & 0.0017 & 2.45 & 2.342 & 0.25 & 0.0449 & 0.0073 & 0.0029 \\ \hline
2.25 & 2.261 & -0.65 & 0.0257 & 0.0223 & 0.0018 & 2.35 & 2.302 & -0.15 & 0.0145 & 0.0069 & 0.0010 & 2.45 & 2.342 & 0.35 & 0.0679 & 0.0091 & 0.0044 \\ \hline
2.25 & 2.261 & -0.55 & 0.0295 & 0.0134 & 0.0021 & 2.35 & 2.302 & -0.05 & 0.0075 & 0.0059 & 0.0005 & 2.45 & 2.342 & 0.45 & 0.1104 & 0.0117 & 0.0072 \\ \hline
2.25 & 2.261 & -0.45 & 0.0372 & 0.0099 & 0.0026 & 2.35 & 2.302 & 0.05 & 0.0175 & 0.0058 & 0.0011 & 2.45 & 2.342 & 0.55 & 0.1625 & 0.0169 & 0.0106 \\ \hline
2.25 & 2.261 & -0.35 & 0.0333 & 0.0081 & 0.0023 &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\end{tabular}}
\end{sideways}
\end{table*}



